Leveraging Learning Metrics for Improved Federated Learning

Currently in the federated setting, no learning schemes leverage the emerging research of explainable artificial intelligence (XAI) in particular the novel learning metrics that help determine how well a model is learning. One of these novel learning metrics is termed `Effective Rank' (ER) which measures the Shannon Entropy of the singular values of a matrix, thus enabling a metric determining how well a layer is mapping. By joining federated learning and the learning metric, effective rank, this work will \textbf{(1)} give the first federated learning metric aggregation method \textbf{(2)} show that effective rank is well-suited to federated problems by out-performing baseline Federated Averaging \cite{konevcny2016federated} and \textbf{(3)} develop a novel weight-aggregation scheme relying on effective rank.

==> ch-future-work.tex <==
\chapter{Future Work}
The next phases are clear for the progression of this work. Firstly, the need to better understand \texttt{Flower}, since the communication framework is complex, is paramount. As this work relies on \texttt{Flower}, this can be completed within a few weeks by re-implementing Federated Averaging \cite{konevcny2016federated}. \\

Secondly, building on this work, the implementation of the quality \& explainability metrics into the work must be done. This is the crux of the research, where the explainability of the client networks, layer-by-layer are evaluated and transmitted, allowing the central server to adjust parameters according to learnings. In this way the expected value of the empirical risk minimization $\mathbb{E}_{\mathcal{D}_k}[F_k(w)] = f(w)$ can be shown to still work in a theoretical bound. \\

Finally, integrating \& testing with existing methods such as precision, unbiased gradient accumulation (UGA) and proximal learning would allow this work to build on the state-of-the-art methods.

\begin{table}[h]
\begin{tabular}{c|l|l|l}
\textbf{Phase} & \multicolumn{1}{c|}{\textbf{Work}}                                             & \multicolumn{1}{c|}{\textbf{Time Estimation}} & \multicolumn{1}{c}{\textbf{Expected Deadline}} \\ \hline
1              & \begin{tabular}[c]{@{}l@{}}Understand Flower \&\\ Build FedAvg\end{tabular}    & 2 weeks                                       & 18 Feb 2022                                    \\ \hline
2              & \begin{tabular}[c]{@{}l@{}}Integrate Explainable \\ Metrics\end{tabular}       & 3 Weeks                                       & 11 March                                       \\ \hline
3              & \begin{tabular}[c]{@{}l@{}}Test SOTA \&\\ Integrate related works\end{tabular} & 2 weeks                                       & 25 March
\end{tabular}
\label{tab:next Steps}
\caption{Next Steps \& Planning calendar}
\end{table}

==> ch-progress.tex <==
\chapter{Progress  To Date}
The first semester was spent mainly setting up the problem statement \& exploring the variety of explainable metrics that can arise. Both Federated Learning \& the explainable AI spaces are extremely vast, and truly understanding the field required time. \\

In recent weeks, the research has progressed significantly, where building the Residual Networks for testing has taken place \& preliminary testing in a federated setting has taken place using \texttt{Flower} \cite{beutel2020flower}, a Federated Learning Framework. \\

The beginnings of the mathematical proof for convergence using explainable metrics has been started as well, allowing theoretical convergence properties to be explored. With the literature review, the precision \& proximal learning can now be included as additional corollaries.



==> tab/quick.tex <==
\begin{tabular}{rl}
  \toprule
  symbol & definition \\
  \midrule
     $x$ & variable   \\
  \bottomrule
\end{tabular}
